Multimodal Foundation Models: From Specialists to General-Purpose Assistants

This paper presents a comprehensive survey of the taxonomy and evolution of multimodal foundation models that demonstrate vision and vision-language capabilities, focusing on the transition from specialist models to general-purpose assistants. The research landscape encompasses five core topics, categorized into two classes. (i) We start with a survey of well-established research areas: multimodal foundation models pre-trained for specific purposes, including two topics -- methods of learning vision backbones for visual understanding and text-to-image generation. (ii) Then, we present recent advances in exploratory, open research areas: multimodal foundation models that aim to play the role of general-purpose assistants, including three topics -- unified vision models inspired by large language models (LLMs), end-to-end training of multimodal LLMs, and chaining multimodal tools with LLMs. The target audiences of the paper are researchers, graduate students, and professionals in computer vision and vision-language multimodal communities who are eager to learn the basics and recent advances in multimodal foundation models.

==> tables/chp3_big_models.tex <==
\begin{table*}[!t]
\resizebox{1.0\textwidth}{!}
{
  \begin{tabular}{l|cccc|c|c}
    %\toprule
    \multirow{2}{*}{\bf Model} & \multicolumn{4}{c|}{\bf Model Size}  & \multirow{2}{*}{\bf PT dataset size}  & \multirow{2}{*}{\bf PT Tasks} \\
    \cmidrule(lr){2-5}
     & Image Enc. & Text Enc.$^\dagger$ & Fusion$^\dagger$ & Total & & \\
    \midrule
  CLIP ViT-L/14~\citep{radford2021learning}  & 302M & 123M & 0 & 425M  & 400M & ITC\\
  ALIGN~\citep{jia2021scaling}  & 480M & 340M & 0  & 820M  & 1.8B & ITC\\
  Florence~\citep{yuan2021florence}  & 637M & 256M & 0  & 893M  & 900M & ITC\\
  \midrule
  SimVLM-huge~\citep{wang2021simvlm}  & 300M & 39M  & 600M  & 939M & 1.8B & PrefixLM\\
  METER-huge~\citep{dou2021empirical}  & 637M & 125M & 220M  & 982M & 900M+20M$^1$ & MLM+ITM\\
  LEMON~\citep{hu2021scaling}  & 147M$^2$ & 39M & 636M  & 822M & 200M & MLM\\
  Flamingo~\citep{alayrac2022flamingo}  & 200M & 70B & 10B  & 80.2B & 2.1B+27M$^3$ & LM\\
  GIT~\citep{wang2022git}  & 637M & 40M & 70M  & 747M & 800M & LM\\
  GIT2~\citep{wang2022git}  & 4.8B & 40M & 260M  & 5.1B & 12.9B & LM\\
  CoCa~\citep{yu2022coca}  & 1B & 477M & 623M  & 2.1B & 1.8B+3B$^4$ & ITC+LM\\
  \multirow{2}{*}{BEiT-3~\citep{wang2022image}}  & \multirow{2}{*}{692M$^5$} & \multirow{2}{*}{692M$^5$} & \multirow{2}{*}{52M$^5$}  & \multirow{2}{*}{1.9B} & \multirow{2}{*}{21M+14M$^6$} & MIM+MLM\\
  & & & & & & +MVLM \\
  \multirow{2}{*}{PaLI~\citep{chen2022pali}}  & \multirow{2}{*}{3.9B} & \multirow{2}{*}{40M} & \multirow{2}{*}{13B}  & \multirow{2}{*}{16.9B} & \multirow{2}{*}{1.6B} & LM+VQA$^7$\\
  & & & & & & +OCR+OD \\
  %\bottomrule
  \end{tabular}
  }
  \caption{\textbf{A summary of recent big VLP models} in terms of model size, pre-training dataset size, and pre-training tasks. Note, that some of the numbers shown in this table are based on our best estimate. $^1$: 20M image-text pairs are used for VLP, while 900M data is used to pre-train the Florence image encoder. $^2$: This is the model size of an object detector as used in VinVL~\citep{zhang2021vinvl}. $^3$: 2.1B image-text data plus 27M video-text data. $^4$: 1.8B image-text data plus 3B image-tag data before filtering. $^5$: shared attention blocks contain another 317M parameters. $^6$: 21M image-text pairs plus 14M images from ImageNet-21K (additional 160GB documents are omitted here). $^7$: A complete set of pre-training tasks for PaLI~\citep{chen2022pali} include LM, PrefixLM, VQA, VQG, OCR, and OD. $^\dagger$: In our context, a module that takes both image and text features as input is considered as the fusion module, and a module that only takes text as input is considered as text encoder. Sometimes, the fusion module is called a text decoder in the literature, such as in SimVLM~\citep{wang2021simvlm}, Flamingo~\citep{alayrac2022flamingo}, and GIT~\citep{wang2022git}. ITC: image-text contrastive loss. ITM: image-text matching. MLM/LM: (masked) language modeling. MIM: masked image modeling. MVLM: masked vision-language modeling. }
  \label{tab:chp3_big_models}
  \vspace{-3mm}
\end{table*}

==> tables/chp3_pretrain_datasets.tex <==
\begin{table}[!t]
%\tablestyle{5pt}{1.0}
%\def\w{25pt} 
%\scalebox{1.0}{
\centering
  \begin{tabular}{c|cccc|c}
    %\toprule
    %\toprule
    & \bf COCO & \bf VG & \bf CC3M & \bf SBU & \bf Total \\
%    \bf Dataset & \bf \#Images & \bf \#Captions \\
    \hline
\#Images & 113K & 108K & 3.1M & 875K & 4.2M\\
\#Captions & 567K & 5.4M & 3.1M & 875K & 10M \\
  %  COCO & 113K & 567K \\
  %  Visual Genome & 108K & 5.4M \\
  %  Conceptual Captions & 3.1M & 3.1M \\
  %  SBU Captions & 875K & 875K \\
    %\bottomrule
  \end{tabular}
%  }
  \caption{Statistics of the pre-training datasets used in a typical academic setting.}
  \label{tab:chp3_vlp_data_stats}
  \vspace{-3mm}
\end{table}

==> tables/chp3_vlp_overview.tex <==
\begin{table*}[!t]
\resizebox{1.0\textwidth}{!}
{
  \begin{tabular}{l|cccc|c}
    %\toprule
    \multirow{2}{*}{\bf Model} & \bf Vision & \bf Text  & \bf Multimodal & \multirow{2}{*}{\bf Decoder} & \bf Pre-training \\
    & \bf Encoder & \bf Encoder  & \bf Fusion &  & \bf Objectives \\
    \hline
    ViLBERT~\citep{lu2019vilbert} & 
\multirow{2}{*}{OD+Xformer}  & \multirow{2}{*}{Xformer}    & \multirow{2}{*}{Co-attn.} &  \multirow{10}{*}{\ding{55}$^\dagger$ } & MLM+ITM+MIM\\
LXMERT~\citep{tan-bansal-2019-lxmert} & &   & &   & MLM+ITM+MIM+VQA \\
    \cdashline{2-4}
    VisualBERT~\citep{li2019visualbert} & \multirow{8}{*}{OD}   & \multirow{8}{*}{Emb.}  & \multirow{8}{*}{Merged-attn.} &    & MLM+ITM\\
 VL-BERT~\citep{su2019vl} &  &  & &    & MLM+MIM\\
  UNITER~\citep{chen2020uniter} & &   & & & MLM+ITM+MIM+WRA \\
  OSCAR~\citep{li2020oscar} & &   & &  & MLM+ITM \\
  VILLA~\citep{gan2020large} & &   & & & MLM+ITM+MIM+WRA \\
  VinVL~\citep{zhang2021vinvl} & &  & &  & MLM+ITM\\
  UNIMO~\citep{li2020unimo} & &  & &  & MLM+ITM+MIM+ITC\\
  \cdashline{5-5}
   VL-T5~\citep{cho2021unifying}  &   &    & & \ding{51} & MLM+ITM+VQA+GC\\
  \hline
  PixelBERT~\citep{huang2020pixel} & \multirow{8}{*}{CNN} & \multirow{4}{*}{Emb.}  & \multirow{7}{*}{Merged-attn.} & \multirow{3}{*}{\ding{55}$^\dagger$ } & MLM+ITM\\
  SOHO~\citep{huang2021seeing} & &  & &  & MLM+ITM+MIM\\
  CLIP-ViL~\citep{shen2021much}  & & & &  & MLM+ITM+VQA\\
  \cdashline{5-5}
   SimVLM~\citep{wang2021simvlm} &   &   &    & \multirow{4}{*}{\ding{51}} & PrefixLM\\
     \cdashline{3-3}
   MDETR~\citep{kamath2021mdetr} &   & \multirow{2}{*}{Xformer} &  & & OD+TP+CA\\
   UniTAB~\citep{yang2021crossing} &  & &  & & Seq2Seq\\
   \cdashline{3-3}
   OFA~\citep{wang2022unifying} &  & \multirow{2}{*}{Emb.} &  & & Seq2Seq\\
   \cdashline{4-5}
   Flamingo~\citep{alayrac2022flamingo} &  &  & Cross-attn. & \ding{55}$^\dagger$  & LM \\
  \hline
  ViLT~\citep{kim2021vilt}& \multirow{1}{*}{Patch Emb.} & \multirow{3}{*}{Emb.}  & \multirow{5}{*}{Merged-attn.} & \multirow{10}{*}{\ding{55}$^\dagger$} & MLM+ITM\\
  \cdashline{2-2}
  Visual Parsing~\citep{xue2021probing} & \multirow{9}{*}{Xformer} &  & &   & MLM+ITM+MIM\\
  GIT~\citep{wang2022git} &  &   &  &  & LM\\
  \cdashline{3-3}
  VLMo~\citep{wang2021vlmo}& & \multirow{7}{*}{Xformer} & & & MLM+ITM+ITC\\
  BEiT-3~\citep{wang2022image}& & & & & MLM+MIM+MVLM\\
  \cdashline{4-4}
  ALBEF~\citep{li2021align} &   &  & \multirow{3}{*}{Cross-attn.} &   & MLM+ITM+ITC\\
  BLIP~\citep{li2022blip} &  &    &  &  & LM+ITM+ITC\\
  CoCa~\citep{yu2022coca} &  &    &  &  & LM+ITC\\
  \cdashline{4-4}
  METER~\citep{dou2021empirical} &  &    & \multirow{2}{*}{Co-attn.} &  & MLM+ITM\\
  FIBER~\citep{dou2022coarse} &  &    &  &  & LM+ITM+ITC\\
  \hline
  CLIP~\citep{radford2021learning}  & CNN/Xformer & \multirow{2}{*}{Xformer} & \multirow{2}{*}{None} &\multirow{2}{*}{\ding{55}}  & \multirow{2}{*}{ITC}\\
  ALIGN~\citep{jia2021scaling}  & CNN & &  &   & \\
  %\bottomrule
  \end{tabular}
  }
  \caption{\textbf{Glossary of representative VLP models}. OD: object detector. Xformer: transformer. Emb.: embedding. MLM/MIM: masked language/image modeling. ITM: image-text matching. ITC: image-text contrastive learning. WRA: word-region alginment.  TP: token prediction. CA: contrastive alignment. GC: grounding+captioning. ($\dagger$) In many cases (\emph{e.g.}, Flamingo~\citep{alayrac2022flamingo}, CoCa~\citep{dou2021empirical}, and GIT~\citep{dou2021empirical}), the multimodal fusion module itself is also directly called (or serves as) the text decoder.}
  \label{tab:chp3_vlp_glossary}
  \vspace{-3mm}
\end{table*}

==> tables/chp4_vlp_for_vision_overview.tex <==
\begin{table*}[!t]
\resizebox{1.0\textwidth}{!}
{
  \begin{tabular}{l|c|ccc|c}
    {\bf Model} & \bf  {\bf Problems}  & \multicolumn{3}{c|}{\bf Pre-training Data}    &    \bf Pre-training Objectives \\ \cline{3-6} 
    \hline
        &    & \bf Image-Text &  \bf Image-label  & \bf Knowledge     & \\        
  CLIP~\citep{radford2021learning}  &\multirow{8}{*}{IC} & WebIT (400M) &  &   & \multirow{2}{*}{ITC}\\
  ALIGN~\citep{jia2021scaling}  &  & WebIT (1.8B) &  &      &\\ \cdashline{6-6}
  FILIP~\citep{yao2021filip}  &  &  YFCC15M, WebIT (300M) &  &     & ITC+WRA\\
  DeCLIP~\citep{li2021supervision}  &  & YFCC15M, WebIT (88M)  &  &      & ITC+SSL+TP\\  
  SLIP~\citep{mu2021slip}  &  & YFCC15M &  &   &    ITC+SSL \\ \cdashline{4-4}\cdashline{6-6}
  Florence~\citep{yuan2021florence}  & &  WebIT 500M & Image-tag 300M &      & \multirow{3}{*}{UniCL} \\   
  UniCL~\citep{yang2022unicl}  &  & CC15M, YFCC15M  &  ImageNet-21K &      &\\   \cdashline{5-5}
  K-Lite~\citep{shen2022k}  &  & CC15M, YFCC15M & ImageNet-21K & Wiktionary, WordNet &    \\  
 \hline
         &    & \bf Image-Text &  \bf OD Annotation & \bf Phrase grounding &   \\   
  ViLD~\citep{gu2021zero}  &\multirow{8}{*}{OD} &  &  LVIS (120K) &   &   \multirow{2}{*}{ITC+ distillation} \\
  RegionCLIP~\citep{zhong2021regionclip}  &  & CC3M &  &   &    \\  \cdashline{6-6}
  GLIP~\citep{li2021grounded}   &  & CC3M+12M,SBU & Combined OD &  Gold-G &     Object-Phrase Alignment\\  
Detic~\citep{zhou2022detecting}  &  & ImageNet & LVIS &   &   Non-prediction-based Loss   \\  
PromptDet~\citep{feng2022promptdet} & & LAION-400M & LVIS &   &   Regional Prompt Learning  \\  
OWL-ViT~\citep{minderer2022simple}   &  & WebIT (3.6B)  & Combined OD (2M) &   &   Bipartite Matching Loss   \\  
OV-DETR~\citep{zang2022open} &  & & COCO / LVIS &   &   Binary Matching Loss \\  
X-DETR~\citep{cai2022x} & & CC,SBU, LocNar & COCO & Gold-G  &  Object-Language Alignment   \\  
% FindIT~\citep{kuo2022findit} &  & &  &   &     
   \hline
           &    & \bf Image-Text &  \bf Seg Annotation  & \bf Phrase grounding  & \\   
  LSeg~\citep{li2022language}  &\multirow{6}{*}{Seg} &   & COCO/VOC &\multirow{3}{*}{}  & Mask Prediction + Grounding  \\
  OpenSeg~\citep{ghiasi2021open}  &  & LocNar & COCO  &     & Word-Pixel Matching \\  
  CLIPSeg~\citep{luddecke2022image}  &  & &   &  PhraseCut  & Visual Prompt Engineering\\ 
  MaskCLIP~\citep{zhou2021maskclip}   &  & &  COCO/VOC &    &  Pseudo Label Distillation\\  
  DenseCLIP~\citep{rao2021denseclip}   &  & & ADE20K/COCO &     & Pixel-Text Matching\\  
  GroupViT~\citep{xu2022groupvit}   &  & CC12M/YFCC15M &  &     & Multi Label Contrastive\\    
  \end{tabular}
  }
  \caption{\textbf{Glossary of representative VLP models for core vision tasks}. For data scale, we report \# image-text pairs, including both image-label and image-caption. IC: image classification. OD: object detection.
  LocNar: Localized Narratives.
  Golden-G is the mixed golden ground-truth grounding data processed in MDETR~\citep{kamath2021mdetr}.
  ITC: image-text contrastive learning. WRA: word-region alignment. TP: Token Prediction. SSL: Self-supervised learning.}
  \label{tab:chp4_core_vision_glossary}
\end{table*}

==> tables/chp5_video_text_overview.tex <==
 \begin{table*}[!t]
\resizebox{1.0\textwidth}{!}
{
  \begin{tabular}{l|lccccc}
    %\toprule
    %\toprule
     \bf \multirow{2}{*}{Model}  & \bf Multimodal & \bf Vision & \bf Text  & \bf \multirow{2}{*}{Decoder} & \bf \multirow{2}{*}{E2E} & \bf Pre-training \\
     & \bf Fusion & \bf Encoder & \bf Encoder & & & \bf Objectives\\
    \hline
VideoBERT~\citep{sun2019videobert} &  & 3D CNN  & Emb.    &  \ding{55} & \ding{55} & MLM+VTM+MVM\\
ActBERT~\citep{zhu2020actbert} &  & OD  & Emb. &  \ding{55}  & \ding{55} & MLM+VTM+MVM\\
% CBT~\citep{sun2019learning}  &  & 3D CNN &   Xformer   &  \ding{55} & \ding{55} & VTC\\
HERO~\citep{li2020hero} &  & 2D+3D CNN & Emb.     &  \ding{55} & \ding{55} & \specialcell{MLM+VTM+FOM\\+MFM}\\
UniVL~\citep{luo2020univl} &  & \specialcell{2D+3D CNN+Xformer} & Xformer  &  \ding{51} & \ding{55} & \specialcell{VTC+MLM+VTM\\+MFM+LM}\\
VQA-T~\citep{yang2021just}  & & 3D CNN & Xformer  &  \ding{55} & \ding{55} & MLM+VTC\\
TACo~\citep{yang2021taco}  & \multirow{1}{*}{Xformer}  & \specialcell{2D+3D CNN} & Xformer     &  \ding{55} & \ding{55} & VTC\\
% VLM~\citep{xu2021vlm} &  & 3D CNN & Emb.   &  \ding{55} & \ding{55} & MLM-MFM+MMM\\
% DeCEMBERT~\citep{tang-etal-2021-decembert} &  & \specialcell{2D+3D CNN} & Emb.    &  \ding{55} & \ding{55} & MLM+VTM+CA\\
\cmidrule(lr){3-7}
ClipBERT~\citep{lei2021less} &  & 2D CNN
  & Emb.  & \ding{55} & \ding{51} & MLM+VTM\\
%  VLM~\citep{xu2021vlm} & \multirow{1}{*}{Xformer} & 3D CNN
%   & Emb.   &  \ding{55} & \ding{55} & MLM-MFM+MMM\\

%   VQA-T~\citep{yang2021just}  &  & \specialcell{3D CNN}
%   & Xformer  &  \ding{55} & \ding{55} & MLM+VTC\\
%   VICTOR~\citep{lei2021understanding}  &  & \specialcell{2D CNN}
%   & Emb.    &  \ding{51} & \ding{55} & \specialcell{MLM+VTC+MFM\\+FOM+SOM+LM}\\
MERLOT~\citep{zellers2021merlot}  &  & \specialcell{2D CNN+Xformer}
& Xformer     &  \ding{55} & \ding{51} & MLM+VTC+FOM\\
MV-GPT~\citep{seo2022end}  &  & Xformer & Emb.     &  \ding{51} & \ding{51} & MLM+LM\\
LAVENDER~\citep{li2022lavender} & & Xformer & Xformer & \ding{55} & \ding{51} & MLM+VTM as MLM\\
Singularity~\citep{lei2022revealing} & & Xformer & Xformer & \ding{55} & \ding{51} & MLM+VTM+VTC\\
% \hline
\midrule

HTM~\citep{miech2019howto100m} &  & 3D CNN  & Word2Vec &  \ding{55} & \ding{51} & VTC\\
MIL-NCE~\citep{miech19endtoend} &  & 3D CNN  & Word2Vec &  \ding{55} & \ding{51} & VTC\\
% MMT~\citep{} &  & 
% \specialcell{2D+3D CNN\\+Xformer}  & \multirow{1}{*}{Xformer}     &  \multirow{1}{*}{\ding{55} } & \ding{55} & VTC\\
    % AVLNet~\citep{} &  & \specialcell{2D+3D CNN} & \multirow{1}{*}{Word2Vec}     &  \multirow{1}{*}{\ding{55} } & \ding{55} & VTC+VAC\\
Support Set~\citep{patrick2020support} & \multirow{1}{*}{Dot Product} & \specialcell{2D+3D CNN+Xformer} & Xformer    &  \ding{51} & \ding{55} & VTC+LM\\
 VideoCLIP~\citep{xu2021videoclip} &  & \specialcell{3D CNN+Xformer} & Xformer   &  \ding{55} & \ding{55} & VTC\\
  Frozen~\citep{bain2021frozen} & & Xformer & Xformer & \ding{55} & \ding{51} & VTC\\
    
%     VATT~\citep{} &  & \specialcell{Xformer}
%   & \multirow{1}{*}{Xformer}     &  \multirow{1}{*}{\ding{55} } & \ding{51} & VTC+VAC\\
  \end{tabular}
  }
  \caption{\textbf{Glossary of representative VLP models for video-text tasks}. E2E: end-to-end. CNN: convolutional neural netowrks. OD: object detector. Xformer: transformer. Emb.: embedding. MLM/MFM/MVM: masked language/frame/video modeling. VTM: video-text matching. VTC: video-text contrastive learning. FOM: frame order modeling. LM: language modeling.
%   SOM: sentence order modeling.  CA: constrained attention loss. 
%   \linjie{Similar to image-text models, add a more complete table to include other works.}
  }
  \label{tab:vlp_glossary_video_text}
\end{table*}

